Data Upcycling Knowledge Distillation for Image Super-Resolution

Knowledge distillation (KD) compresses deep neural networks by transferring task-related knowledge from cumbersome pre-trained teacher models to compact student models. However, current KD methods for super-resolution (SR) networks overlook the nature of SR task that the outputs of the teacher model are noisy approximations to the ground-truth distribution of high-quality images (GT), which shades the teacher model's knowledge to result in limited KD effects. To utilize the teacher model beyond the GT upper-bound, we present the Data Upcycling Knowledge Distillation (DUKD), to transfer the teacher model's knowledge to the student model through the upcycled in-domain data derived from training data. Besides, we impose label consistency regularization to KD for SR by the paired invertible augmentations to improve the student model's performance and robustness. Comprehensive experiments demonstrate that the DUKD method significantly outperforms previous arts on several SR tasks.

==> figure/visualization/realworld/realworld.tex <==
\begin{figure*}[h]
	\resizebox{\linewidth}{!}{%
		\setlength{\abovecaptionskip}{0.cm}
		\setlength{\belowcaptionskip}{-0.cm}
		\centering
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_001}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}			
		\end{minipage}
		\begin{minipage}{0.12\linewidth}			
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_001}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_001}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_001}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_001}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
		
		
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_016}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_016}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_016}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_016}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_016}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
		
		
		
		
	} %
	
	
	\resizebox{\linewidth}{!}{%
		\setlength{\abovecaptionskip}{0.cm}
		\setlength{\belowcaptionskip}{-0.cm}
		\centering
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_021}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_021}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_021}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_021}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_021}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
		
		
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_025}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_025}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_025}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_025}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_025}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
	}
	
	\resizebox{\linewidth}{!}{%
		\setlength{\abovecaptionskip}{0.cm}
		\setlength{\belowcaptionskip}{-0.cm}
		\centering
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_041}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_041}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_041}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_041}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_041}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
		
		\begin{minipage}{0.24\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/Nikon\_044}
				\put(1.5,90){\tcbox{\scriptsize Input}}
			\end{overpic}
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/teacher_Nikon\_044}
				\put(2.5,80){\tcbox{\scriptsize Teacher}}
			\end{overpic}		
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/kd_Nikon\_044}
				\put(2.5,80){\tcbox{\scriptsize KD}}
			\end{overpic}		
		\end{minipage}
		\begin{minipage}{0.12\linewidth}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/scratch_Nikon\_044}
				\put(2.5,80){\tcbox{\scriptsize Scratch}}
			\end{overpic}
			\begin{overpic}[width=\linewidth]{figure/visualization/realworld/dukd_Nikon\_044}
				\put(2.5,80){\tcbox{\scriptsize DUKD}}
			\end{overpic}
			
		\end{minipage}
	}
	
	
	\caption{Visual comparisons on several representative real-world samples of \texttimes 4 SR scale. DUKD outperforms other approaches in removing artifacts and restoring details, and its outputs are more similar with the teacher model's. Zoom in~\faSearchPluss~for the best view.}
	
	\label{fig:vis_real}
\end{figure*}

